Detections of millisecond pulsars with the Fermi Large Area Telescope

The Fermi observatory was launched on June 11, 2008. It hosts the \emph{Large Area Telescope} (LAT), sensitive to $\gamma$-ray photons from 20 MeV to over 300 GeV. When the LAT began its activity, nine young and energetic pulsars were known in $\gamma$ rays. At least several tens of pulsar detections by the LAT were predicted before launch. The LAT also allowed the study of millisecond pulsars (MSPs), never firmly detected in $\gamma$ rays before Fermi. This thesis first presents the pulsar timing campaign for the LAT, in collaboration with large radiotelescopes and X-ray telescopes, allowing for high sensitivity pulsed searches. Furthermore, it lead to quasi-homogeneous coverage of the galactic MSPs, so that the search for pulsations in LAT data for this population of stars was not affected by an \emph{a priori} bias. We present a search for pulsations from these objects in LAT data. For the first time, eight galactic MSPs have been detected as sources of pulsed $\gamma$-ray emission over 100 MeV. In addition, a couple of good candidates for future detection are seen. A similar search for globular cluster MSPs has not succeeded so far. Comparison of the phase-aligned $\gamma$-ray and radio light curves, as well as the spectral shapes, leads to the conclusion that their $\gamma$-ray emission is similar to that of normal pulsars, and is probably produced in the outer-magnetosphere. This discovery suggests that many unresolved $\gamma$-ray sources are unknown MSPs.

==> figures/chap1/GL_GB_Distance.tex <==
\subfigure[Latitude galactique $b$ en fonction de la distance]{\includegraphics[scale=0.75]{figures/chap1/GB_Dist1.pdf}}
\subfigure[Les pulsars connus en coordonnées galactiques]{\includegraphics[scale=0.75]{figures/chap1/GL_GB.pdf}}


==> figures/chap1/masserayon.tex <==
\subfigure[Modèles d'équation d'état de la matière des étoiles à neutrons]{\includegraphics[width=10cm]{figures/chap1/lattimer_fig2.pdf}}
\subfigure[Relations masse-rayon pour différentes valeurs du moment d'inertie]{\includegraphics[width=10cm]{figures/chap1/inertia.pdf}}


==> figures/chap3/TimingCorrections.tex <==
\subfigure[Erreur sur la fréquence de rotation $f_0$]{\includegraphics[scale=0.5]{figures/chap3/0030_badF0.pdf}}
\subfigure[Erreur sur la dérivée première de la fréquence, $\dot f_0$]{\includegraphics[scale=0.5]{figures/chap3/0030_badF1.pdf}}
\subfigure[Mauvaise position du pulsar]{\includegraphics[scale=0.5]{figures/chap3/0030_badpos.pdf}}
\subfigure[Mouvement propre du pulsar non pris en compte]{\includegraphics[scale=0.5]{figures/chap3/0030_noPM.pdf}}


==> figures/chap3/TimingNoiseCrabe.tex <==
\subfigure[Modèle de datation limité à $f_0$,$\dot f_0$ et $\ddot f_0$]{\includegraphics[scale=0.67]{figures/chap3/ResidusCrabe_bad.pdf}}
\subfigure[Emploi d'un développement en harmoniques]{\includegraphics[scale=0.67]{figures/chap3/ResidusCrabe_good.pdf}}

==> figures/chap3/gp1937.tex <==
\subfigure[GRPs de B1937+21 sur l'ensemble de la rotation]{\includegraphics[scale=0.5]{figures/chap3/gp1937_good.pdf}}
\subfigure[Zoom sur la composante principale de l'émission]{\includegraphics[scale=0.5]{figures/chap3/gp1937_zoom_good.pdf}}

==> figures/chap5/phasos1.tex <==
\subfigure[J0030+0451]{\includegraphics[scale=0.37]{figures/chap5/0030p0451_2.pdf}}
\subfigure[J0218+4232]{\includegraphics[scale=0.37]{figures/chap5/0218p4232_2.pdf}}
\subfigure[J0437$-$4715]{\includegraphics[scale=0.37]{figures/chap5/0437m4715_2.pdf}}
\subfigure[J0613$-$0200]{\includegraphics[scale=0.37]{figures/chap5/0613m0200_2.pdf}}


==> figures/chap5/phasos2.tex <==
\subfigure[J0751+1807]{\includegraphics[scale=0.37]{figures/chap5/0751p1807_2.pdf}}
\subfigure[J1614$-$2230]{\includegraphics[scale=0.37]{figures/chap5/1614m2230_2.pdf}}
\subfigure[J1744$-$1134]{\includegraphics[scale=0.37]{figures/chap5/1744m1134_2.pdf}}
\subfigure[J2124$-$3358]{\includegraphics[scale=0.37]{figures/chap5/2124m3358_2.pdf}}


==> figures/chap5/phasos_0034_1713.tex <==
\subfigure[J0034$-$0534]{\includegraphics[scale=0.37]{figures/chap5/0034m0534_2.pdf}}
\subfigure[J1713+0747]{\includegraphics[scale=0.37]{figures/chap5/1713p0747_2.pdf}}

==> figures/chap5/prog_lin2.tex <==
\subfigure[J0034$-$0534]{\includegraphics[width=10cm]{figures/chap5/0034-0534.pdf}}
\subfigure[J1713+0747]{\includegraphics[width=10cm]{figures/chap5/1713+0747.pdf}}

==> figures/chap5/spectres.tex <==
\subfigure[J0030+0451]{\includegraphics[width=12cm]{figures/chap5/Lucas_J0030_SED_noBT.pdf}}
\subfigure[J1614$-$2230]{\includegraphics[width=12cm]{figures/chap5/Lucas_J1614_SED.pdf}}

==> figures/chap5/tendances.tex <==
\subfigure[$\Gamma$ en fonction de $\tau$]{\includegraphics[scale=0.67]{figures/chap5/AgeIndex.pdf}}
\subfigure[$E_c$ en fonction de $B_S$]{\includegraphics[scale=0.67]{figures/chap5/BsurfCutoff.pdf}}

==> tableaux/EGRETpsrs.tex <==
\begin{scriptsize}
\begin{tabular}{lccccccccc}
\hline
\hline
Nom & P$_0$ & \^{A}ge & log($\dot E$) & Distance & $\Gamma$ & E$_0$ & $f$ (> 100 MeV) & $h$ (> 100 MeV) & $\eta$ (> 100 MeV) \\
    & (s) & (10$^3$ yr) & (erg/s) & (kpc) & & (GeV) & (/cm$^2$/s) & (erg/cm$^2$/s) & \\
\hline
Crabe      & 0.033 & 1.24 & 38.7 & 2.0 $\pm$ 0.2             & x & x & x & x & x \\
Vela       & 0.089 & 11.3 & 36.8 & 0.287$_{-0.017}^{+0.019}$ & x & x & x & x & x \\
Geminga    & 0.237 & 342  & 34.5 & 0.25$_{-0.062}^{+0.012}$  & x & x & x & x & x \\
B1055$-$52 & 0.197 & 535  & 34.5 & 0.72 $\pm$ 0.15           & x & x & x & x & x \\
B1509$-$58 & 0.150 & 1.55 & 37.2 & 4.22 $\pm$ 0.6            & x & x & x & x & x \\
B1706$-$44 & 0.102 & 17.5 & 36.5 & 2.3 $\pm$ 0.7             & x & x & x & x & x \\
B1951+32   & 0.039 & 107  & 36.6 & 2.0 $\pm$ 0.6             & x & x & x & x & x \\
\hline
\end{tabular}
\end{scriptsize}

==> tableaux/LATPerformances.tex <==
\begin{scriptsize}
\begin{tabular}{lc}
\hline
\hline
Paramètre & Valeur \\
\hline
Dimensions & 1,8 $\times$ 1,8 $\times$ 0,72 m$^3$ \\
Masse totale & 2789 kg \\
 & \\
Gamme d'énergie & 20 MeV -- 300 GeV \\
Surface effective maximale à incidence normale & 9500 cm$^2$ \\
Champ de vue & 2,4 sr \\
Temps mort & 26,5 $\mu$s \\
Précision en temps & $<$ 1 $\mu$s \\
 & \\
\emph{Résolution en énergie (incidence normale) :} & \\
100 MeV -- 1 GeV & 9\% -- 15\% \\
1 GeV -- 10 GeV & 8\% -- 9\% \\
$\geq$ 10 GeV & 8,5\% -- 18\% \\
 & \\
\emph{Résolution angulaire (incidence normale, 68\% de la PSF) :} & \\
100 MeV & 3,5$^\circ$ \\
1 GeV & 0,6$^\circ$ \\
$>$ 10 GeV & $\leq$ 0,15$^\circ$ \\
\hline
\end{tabular}
\end{scriptsize}


==> tableaux/TS_MSPs.tex <==
\begin{scriptsize}
\begin{tabular}{ccc}
\hline
\hline
Pulsar & $TS$ & Détection pulsée ? \\
       &      &                    \\
\hline
J0030+0451 & 1232,7 & $p$ \\
J0034$-$0534 & 196,1 & $m$ \\
J0218+4232 & 278,0 & $p$ \\
J0437$-$4715 & 189,4 & $p$ \\
J0610$-$2100 & 61,6 & \\
J0613$-$0200 & 310,3 & $p$ \\
J0621+1002 & 59,3 & \\
J0751+1807 & 211,4 & $p$ \\
J1600$-$3053 & 35,7 & \\
J1614$-$2230 & 188,6 & $p$ \\
J1713+0747 & 75,5 & $m$ \\
J1744$-$1134 & 196,3 & $p$ \\
J1939+2134 & 99,8 & \\
J1959+2048 & 64,5 & \\
J2124$-$3358 & 571,3 & $p$ \\
\hline
\end{tabular}
\end{scriptsize}

==> tableaux/coupuresC.tex <==
\begin{scriptsize}
\begin{center}
\begin{tabular}{ccccccc}
\hline
\hline
 & & & \multicolumn{4}{c}{Niveaux de fond} \\
Pulsar & PSF & Note & $>$ 100 MeV & 100 -- 300 MeV & 300 -- 1000 MeV & $>$ 1 GeV \\
\hline
J0030+0451 & 68\% & & 984 (19,7) & 784 (15,7) & 193 (3,9) & 4 (0,1) \\
J0218+4232 & 33\% & Blazar 3C 66A à 1$^\circ$ & 575 (25) & 420 (16,8) & 125 (5) & 5 (0,2) \\
J0437$-$4715 & 68\% & & 760 (30,4) & 638 (25,5) & 120 (4,8) & 3 (0,1) \\
J0613$-$0200 & 68\% & & 2632 (105,3) & 2044 (81,8) & 570 (22,8) & 26 (1) \\
J0751+1807 & 33\% & Blazar PKS 0735+17 à 3$^\circ$ & 322 (12,9) & 274 (11,0) & 56 (2,2) & 0 (0) \\
J1614$-$2230 & 33\% & Région bruitée & 747 (29,9) & 587 (23,5) & 153 (6,1) & 7 (0,3) \\
J1744$-$1134 & 33\% & Région bruitée & 1623 (64,9) & 1265 (50,6) & 347 (13,9) & 18 (0,7) \\
J2124$-$3358 & 68\% & & 1227 (49,1) & 937 (37,5) & 285 (11,4) & 13 (0,5) \\ 
\hline
\end{tabular}
\end{center}
\end{scriptsize}


==> tableaux/ephemGC.tex <==
\begin{scriptsize}
\begin{center}
\begin{tabular}{ccc}
\hline
\hline
Pulsar & Amas globulaire & Observatoire \\
\hline
J1518+0204A & M5 (NGC 5904) & Nançay \\
J1623$-$2631 & M4 (NGC 6121) & Nançay, Jodrell Bank \\
J1641+3627A & M13 (NGC 6205) & Nançay, Green Bank \\
J1701$-$3006A & M65 (NGC 6266) & Nançay \\
J1721$-$1936 & NGC 6342 & Jodrell Bank \\
J1748$-$2446A & Terzan 5 & Nançay, Jodrell Bank \\
J1748$-$2446C & Terzan 5 & Jodrell Bank \\
J1748$-$2021A & NGC 6440 & Jodrell Bank \\
J1804$-$0735 & NGC 6539 & Jodrell Bank \\
J1807$-$2459A & NGC 6544 & Nançay, Jodrell Bank \\
J1823$-$3021A & NGC 6624 & Nançay, Jodrell Bank \\
J1823$-$3021B & NGC 6624 & Nançay, Jodrell Bank \\
J1824$-$2452A & M28 (NGC 6626) & Nançay, Jodrell Bank \\
J2129+1210A & M15 (NGC 7078) & Nançay \\
J2140$-$2310A & M30 (NGC 7099) & Nançay \\
\hline
\end{tabular}
\end{center}
\end{scriptsize}

==> tableaux/nondetections.tex <==
\begin{scriptsize}
\begin{tabular}{ccccc}
\hline
\hline
Pulsar & $P$ & $\dot E$ & Distance & Référence \\
 & (ms) & ($10^{33}$ erg/s) & (kpc) & \\
\hline
J1012+5307 & 5,256 & 3,7 & 0,41 & NE2001 \citep{NE2001} \\
J1024$-$0719 & 5,162 & 5,318 & 0,52 & \citet{Hotan2006} \\
%J1741+1354 & 3,747 & -- & 0,9 & NE2001 (Cordes \& Lazio 2001) \\
J1843$-$1113 & 1,846 & 60,2 & 1,69 & NE2001 \citep{NE2001} \\
J1909$-$3744 & 2.947 & 4,1 & 1,14 &  \citet{Hotan2006} \\
J1911$-$1114 & 3,626 & 7 & 1,22 & NE2001 \citep{NE2001} \\
J1933$-$6211 & 3,543 & 3,28 & 0,52 & NE2001 \citep{NE2001} \\
J2129$-$5721 & 3,726 & 22,1 & 1,36 & NE2001 \citep{NE2001} \\
\hline
\end{tabular}
\end{scriptsize}

==> tableaux/spectres.tex <==
\begin{scriptsize}
\begin{tabular}{ccccccccc}
\hline
\hline
Pulsar & $P$ & $\delta$ & $\Delta$ & $f\ (\mathrm{> 100\ MeV})$ & $h\ (\mathrm{> 100\ MeV})$ & $\Gamma$ & $E_c$ & $L_\gamma$ \\
           & (ms) & & & (10$^{-8}$  & (10$^{-11}$ & & (GeV) & ($10^{32}$ erg/s) \\
           & & & & ph/cm$^2$/s) & erg/cm$^2$/s) & & &  \\
\hline
J0030+0451 & 4,865 & 0,16 & 0,45 & 5,5 $\pm$ 0,7 & 4,9 $\pm$ 0,3 & 1,3 $\pm$ 0,2 & 1,9 $\pm$ 0,4 & 5,3$_{-1,7}^{+2,8}$\\
J0218+4232 & 2,323 & 0,5 & -- & 5,6 $\pm$ 1,3 & 3,5 $\pm$ 0,5 & 2,0 $\pm$ 0,2 & 7 $\pm$ 4 & (3,0 $\pm$ 0,9) $\times 10^2$\\
J0437$-$4715 & 5,757 & 0,45 & -- & 4,4 $\pm$ 1,0 & 1,9 $\pm$ 0,3 & 2,1 $\pm$ 0,3 & 2,1 $\pm$ 1,1 & 0,56 $\pm$ 0,09\\
J0613$-$0200 & 3,062 & 0,42 & -- & 3,1 $\pm$ 0,7 & 3,1 $\pm$ 0,3 & 1,4 $\pm$ 0,2 & 2,9 $\pm$ 0,7 & 8,4$_{-2,9}^{+4,8}$\\
J0751+1807 & 3,479 & 0,5 & -- & 2,0 $\pm$ 0,7 & 1,7 $\pm$ 0,2 & 1,6 $\pm$ 0,2 & 3,4 $\pm$ 1,2 & 7,7$_{-3,8}^{+10,9}$\\
J1614$-$2230 & 3,151 & 0,2 & 0,5 & 2,3 $\pm$ 2,1 & 2,5 $\pm$ 0,8 & 1,0 $\pm$ 0,3 & 1,2 $\pm$ 0,5 & 50 $\pm$ 22\\
J1744$-$1134 & 4,075 & 0,85 & -- & 7,1 $\pm$ 1,4 & 4,0 $\pm$ 1,0 & 1,5 $\pm$ 0,2 & 1,1 $\pm$ 0,2 & 11$_{-4}^{+5}$\\
J2124$-$3358 & 4,931 & 0,85 & -- & 2,9 $\pm$ 0,5 & 3,4 $\pm$ 0,3 & 1,3 $\pm$ 0,2 & 2,9 $\pm$ 0,9 & 2,5$_{-1,2}^{+3,6}$\\
\hline
\end{tabular}
\end{scriptsize}
